A Digital Twin Framework for Physical-Virtual Integration in V2X-Enabled Connected Vehicle Corridors

Transportation Cyber-Physical Systems (T-CPS) enhance safety and mobility by integrating cyber and physical transportation systems. A key component of T-CPS is the Digital Twin (DT), a virtual representation that enables simulation, analysis, and optimization through real-time data exchange and communication. Although existing studies have explored DTs for vehicles, communications, pedestrians, and traffic, real-world validations and implementations of DTs that encompass infrastructure, vehicles, signals, communications, and more remain limited due to several challenges. These include accessing real-world connected infrastructure, integrating heterogeneous, multi-sourced data, ensuring real-time data processing, and synchronizing the digital and physical systems. To address these challenges, this study develops a traffic DT based on a real-world connected vehicle corridor. Leveraging the Cellular Vehicle-to-Everything (C-V2X) infrastructure in the corridor, along with communication, computing, and simulation technologies, the proposed DT accurately replicates physical vehicle behaviors, signal timing, communications, and traffic patterns within the virtual environment. Building upon the previous data pipeline, the digital system ensures robust synchronization with the physical environment. Moreover, the DT's scalable and redundant architecture enhances data integrity, making it capable of supporting future large-scale C-V2X deployments. Furthermore, its ability to provide feedback to the physical system is demonstrated through applications such as signal timing adjustments, vehicle advisory messages, and incident notifications. The proposed DT is a vital tool in T-CPS, enabling real-time traffic monitoring, prediction, and optimization to enhance the reliability and safety of transportation systems.

==> ref.tex <==
\bibitem{xiong2015cyber}Xiong, G., Zhu, F., Liu, X., Dong, X., Huang, W., Chen, S. \& Zhao, K. Cyber-physical-social system in intelligent transportation. {\em IEEE/CAA Journal Of Automatica Sinica}. \textbf{2}, 320-333 (2015)

\bibitem{rawat2015towards}Rawat, D., Bajracharya, C. \& Yan, G. Towards intelligent transportation cyber-physical systems: Real-time computing and communications perspectives. {\em SoutheastCon 2015}. pp. 1-6 (2015)

\bibitem{ran2019development}Ran, B., Cheng, Y., Leight, S. \& Parker, S. Development of an integrated transportation system of connected automated vehicles and highways. {\em ITE Journal}. \textbf{89} (2019)

\bibitem{Joshua2017}Auld, J., Sokolov, V. \& Stephens, T. Analysis of the Effects of Connected–Automated Vehicle Technologies on Travel Demand. {\em Transportation Research Record}. \textbf{2625}, 1-8 (2017), https://doi.org/10.3141/2625-01

\bibitem{saroj2021development}Saroj, A., Roy, S., Guin, A. \& Hunter, M. Development of a connected corridor real-time data-driven traffic digital twin simulation model. {\em Journal Of Transportation Engineering, Part A: Systems}. \textbf{147}, 04021096 (2021)


\bibitem{chowdhury2018}Chowdhury, M., Rahman, M., Rayamajhi, A., Khan, S., Islam, M., Khan, Z. \& Martin, J. Lessons learned from the real-world deployment of a connected vehicle testbed. {\em Transportation Research Record}. \textbf{2672}, 10-23 (2018)

\bibitem{deployment2017}Deployment, S. P. M. Lessons Learned and Recommendations for Future Connected Vehicle Activities. {\em FHWA-JPO-16-363}. (2017)

\bibitem{wu2023development}Wu, K., Cheng, Y., Parker, S., Ran, B. \& Noyce, D. Development of the Data Pipeline for a Connected Vehicle Corridor. {\em International Conference On Transportation And Development 2023}. pp. 218-230 (2023)

\bibitem{li2023does}Li, P., Wu, K., Cheng, Y., Parker, S. \& Noyce, D. How does c-v2x perform in urban environments? results from real-world experiments on urban arterials. {\em IEEE Transactions On Intelligent Vehicles}. (2023)

\bibitem{you2024v2x}You, J., Shi, H., Jiang, Z., Huang, Z., Gan, R., Wu, K., Cheng, X., Li, X. \& Ran, B. V2X-VLM: End-to-End V2X Cooperative Autonomous Driving Through Large Vision-Language Models. {\em ArXiv Preprint ArXiv:2408.09251}. (2024)

\bibitem{farrell2015}Farrell, J. \& Barth, M. Precision Mapping of the California Connected Vehicle Testbed Corridor.  (2015)

\bibitem{feng2019}Feng, Y., Bao, S. \& Liu, H. Connected and Automated Vehicle (CAV) Testing Scenario Design and Implementation Using Naturalistic Driving Data and Augmented Reality. (University of Michigan Transportation Research Institute,2019)

\bibitem{tajalli2021networklevel}Tajalli, M., Mehrabipour, M. \& Hajbabaie, A. Network-Level Coordinated Speed Optimization and Traffic Light Control for Connected and Automated Vehicles. {\em IEEE Transactions On Intelligent Transportation Systems}. (2021)

\bibitem{Souza2019}Souza, V., Cruz, R., Silva, W., Lins, S. \& Lucena, V. A Digital Twin Architecture Based on the Industrial Internet of Things Technologies. {\em 2019 IEEE International Conference On Consumer Electronics (ICCE)}. pp. 1-2 (2019)

\bibitem{Almeaibed2021}Almeaibed, S., Al-Rubaye, S., Tsourdos, A. \& Avdelidis, N. Digital Twin Analysis to Promote Safety and Security in Autonomous Vehicles. {\em IEEE Communications Standards Magazine}. \textbf{5}, 40-46 (2021)

\bibitem{Wang2022}Wang, Z., Gupta, R., Han, K., Wang, H., Ganlath, A., Ammar, N. \& Tiwari, P. Mobility Digital Twin: Concept, Architecture, Case Study, and Future Challenges. {\em IEEE Internet Of Things Journal}. \textbf{9}, 17452-17467 (2022)

\bibitem{hui2022collaboration}Hui, Y., Ma, X., Su, Z., Cheng, N., Yin, Z., Luan, T. \& Chen, Y. Collaboration as a service: Digital-twin-enabled collaborative and distributed autonomous driving. {\em IEEE Internet Of Things Journal}. \textbf{9}, 18607-18619 (2022)


\bibitem{niaz2021autonomous}Niaz, A., Shoukat, M., Jia, Y., Khan, S., Niaz, F. \& Raza, M. Autonomous driving test method based on digital twin: A survey. {\em 2021 International Conference On Computing, Electronic And Electrical Engineering (ICE Cube)}. pp. 1-7 (2021)

\bibitem{hu2022review}Hu, Z., Lou, S., Xing, Y., Wang, X., Cao, D. \& Lv, C. Review and perspectives on driver digital twin and its enabling technologies for intelligent vehicles. {\em IEEE Transactions On Intelligent Vehicles}. (2022)

\bibitem{gao2021digital}Gao, Y., Qian, S., Li, Z., Wang, P., Wang, F. \& He, Q. Digital twin and its application in transportation infrastructure. {\em 2021 IEEE 1st International Conference On Digital Twins And Parallel Intelligence (DTPI)}. pp. 298-301 (2021)

\bibitem{martinez2021digital}Mart\'inez-Guti\'errez, A., Dı\'iez-Gonz\'alez, J., Ferrero-Guill\'en, R., Verde, P., \'Alvarez, R. \& Perez, H. Digital twin for automatic transportation in industry 4.0. {\em Sensors}. \textbf{21}, 3344 (2021)

\bibitem{ye2023developing} Ye, X., Du, J., Han, Y., Newman, G., Retchless, D., Zou, L., Ham, Y., \& Cai, Z. (2023). Developing human-centered urban digital twins for community infrastructure resilience: A research agenda. {\em Journal of Planning Literature}, 38(2), 187-199.

% \bibitem{azfar2022efficient}Azfar, T., Weidner, J., Raheem, A., Ke, R. \& Cheu, R. Efficient procedure of building university campus models for digital twin simulation. {\em IEEE Journal Of Radio Frequency Identification}. \textbf{6} pp. 769-773 (2022)


\bibitem{cai2023}Cai, G., Fan, B., Dong, Y., Li, T., Wu, Y. \& Zhang, Y. Task-Efficiency Oriented V2X Communications: Digital Twin Meets Mobile Edge Computing. {\em IEEE Wireless Communications}. pp. 1-8 (2023)

\bibitem{WAGNER2023}Wágner, T., Ormándi, T., Tettamanti, T. \& Varga, I. SPaT/MAP V2X communication between traffic light and vehicles and a realization with digital twin. {\em Computers And Electrical Engineering}. \textbf{106} pp. 108560 (2023)

\bibitem{you2024realworlddatainspiredinteractive}You, J., Li, P., Cheng, Y., Wu, K., Gan, R., Parker, S. \& Ran, B. Real-World Data Inspired Interactive Connected Traffic Scenario Generation.  (2024), https://arxiv.org/abs/2409.17429


\bibitem{Schwarz2022}Schwarz, C. \& Wang, Z. The Role of Digital Twins in Connected and Automated Vehicles. {\em IEEE Intelligent Transportation Systems Magazine}. \textbf{14}, 41-51 (2022)

\bibitem{VANDERHORN2021113524}VanDerHorn, E. \& Mahadevan, S. Digital Twin: Generalization, characterization and implementation. {\em Decision Support Systems}. \textbf{145} pp. 113524 (2021), https://www.sciencedirect.com/science/article/pii/S0167923621000348

\bibitem{dosovitskiy2017carla}Dosovitskiy, A., Ros, G., Codevilla, F., Lopez, A. \& Koltun, V. CARLA: An open urban driving simulator. {\em Conference On Robot Learning}. pp. 1-16 (2017)

\bibitem{chen2021hierarchical}Chen, N., Arem, B., Alkim, T. \& Wang, M. A Hierarchical Model-Based Optimization Control Approach for Cooperative Merging by Connected Automated Vehicles. {\em IEEE Transactions On Intelligent Transportation Systems}. (2021)

\bibitem{sae2016dsrc}SAE Dedicated Short Range Communications (DSRC) Message Set Dictionary. (SAE International,2016)

\bibitem{kenney2011dsrc}Kenney, J. Dedicated short-range communications (DSRC) standards in the United States. {\em Proceedings Of The IEEE}. \textbf{99}, 1162-1182 (2011)

\bibitem{convexhull}Liu, K. \& Wang, J. Fast Dynamic Vehicle Detection in Road Scenarios Based on Pose Estimation with Convex-Hull Model. {\em Sensors}. \textbf{19} (2019), https://www.mdpi.com/1424-8220/19/14/3136

\bibitem{hang2021cooperative}Hang, P., Lv, C., Huang, C., Xing, Y. \& Hu, Z. Cooperative Decision Making of Connected Automated Vehicles at Multi-Lane Merging Zone: A Coalitional Game Approach. {\em IEEE Transactions On Intelligent Transportation Systems}. (2021)

\bibitem{parker2006wistransportal}Parker, S. \& Tao, Y. WisTransPortal: a Wisconsin traffic operations data hub. {\em Applications Of Advanced Technology In Transportation}. pp. 611-616 (2006)

% \bibitem{wang2023new}Wang, Z., Lv, C. \& Wang, F. A new era of intelligent vehicles and intelligent transportation systems: Digital twins and parallel intelligence. {\em IEEE Transactions On Intelligent Vehicles}. \textbf{8}, 2619-2627 (2023)

% \bibitem{wang2021digital}Wang, Z., Han, K. \& Tiwari, P. Digital twin simulation of connected and automated vehicles with the unity game engine. {\em 2021 IEEE 1st International Conference On Digital Twins And Parallel Intelligence (DTPI)}. pp. 1-4 (2021)

\bibitem{sae-j2735_2016}
SAE International, ``Dedicated Short Range Communications (DSRC) Message Set Dictionary,'' SAE Standard J2735\_201603, March 2016. [Online]. Available: \url{https://www.sae.org/standards/content/j2735_201603/}.























